Distributed Extra-gradient with Optimal Complexity and Communication Guarantees

We consider monotone variational inequality (VI) problems in multi-GPU settings where multiple processors/workers/clients have access to local stochastic dual vectors. This setting includes a broad range of important problems from distributed convex minimization to min-max and games. Extra-gradient, which is a de facto algorithm for monotone VI problems, has not been designed to be communication-efficient. To this end, we propose a quantized generalized extra-gradient (Q-GenX), which is an unbiased and adaptive compression method tailored to solve VIs. We provide an adaptive step-size rule, which adapts to the respective noise profiles at hand and achieve a fast rate of ${\mathcal O}(1/T)$ under relative noise, and an order-optimal ${\mathcal O}(1/\sqrt{T})$ under absolute noise and show distributed training accelerates convergence. Finally, we validate our theoretical results by providing real-world experiments and training generative adversarial networks on multiple GPUs.

==> defsSlides.tex <==

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max} \DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\diag}{diag} \DeclareMathOperator{\bdiag}{bdiag}\DeclareMathOperator{\Real}{\Re}
\DeclareMathOperator{\SNR}{SNR}\DeclareMathOperator{\SINR}{SINR}
\DeclareMathOperator{\nulls}{null}
\newcommand{\ud}{\,\mathrm{d}}
\newcommand{\ENCODE}{\mathrm{ENCODE}}
\newcommand{\DECODE}{\mathrm{DECODE}}
\newcommand{\Elias}{\mathrm{ERC}}

\def \l{\left}
\def \r{\right}
\def \a{\alpha}
\def \b{\beta}
\def \g{\gamma}
\def \z{\zeta}
\def\o{\omega}
\def \t{\tau}
\def \s{\sigma}
\def \eps{\epsilon}
\def\dag{{\cal y}}
\def\reals{\mathbb{R}}
\def\complex{\mathbb{C}}
\def\integers{\mathbb{Z}}
\def\alphabf{\boldsymbol \alpha}
\def\betabf{\boldsymbol \beta }
\def\gammabf{\boldsymbol \gamma }
\def\deltabf{\boldsymbol \delta }
\def\epsilonbf{\boldsymbol \epsilon }
\def\zetabf{\boldsymbol \zeta }
\def\etabf{\boldsymbol \eta }
\def\iotabf{\boldsymbol \iota }
\def\kappabf{\boldsymbol \kappa }
\def\lambdabf{\boldsymbol \lambda }
\def\mubf{\boldsymbol \mu }
\def\nubf{\boldsymbol \nu }
\def\xibf{\boldsymbol \xi }
\def\pibf{\boldsymbol \pi }
\def\rhobf{\boldsymbol \rho }
\def\sigmabf{\boldsymbol \sigma }
\def\taubf{\boldsymbol \tau }
\def\upsilonbf{\boldsymbol \upsilon }
\def\phibf{\boldsymbol \phi }
\def\chibf{\boldsymbol \chi }
\def\psibf{\boldsymbol \psi }
\def\omegabf{\boldsymbol \omega }
\def\Sigmabf{\boldsymbol \Sigma}
\def\Upsilonbf{\boldsymbol \Upsilon}
\def\Phibf{\boldsymbol \Phi}
\def\Psibf{\boldsymbol \Psi}
\def\Omegabf{\boldsymbol \Omega}
\def\Deltabf{\boldsymbol \Delta}
\def\Gammabf{\boldsymbol \Gamma}
\def\Thetabf{\boldsymbol \Theta}
\def\Lambdabf{\boldsymbol \Lambda}
\def\Xibf{\boldsymbol \Xi}
\def\Pibf{{\bf \Pi}}
\def\abf{{\bf a}}
\def\bbf{{\bf b}}
\def\cbf{{\bf c}}
\def\dbf{{\bf d}}
\def\ebf{{\bf e}}
\def\fbf{{\bf f}}
\def\gbf{{\bf g}}
\def\hbf{{\bf h}}
\def\ibf{{\bf i}}
\def\jbf{{\bf j}}
\def\kbf{{\bf k}}
\def\lbf{{\bf l}}
\def\mbf{{\bf m}}
\def\nbf{{\bf n}}
\def\obf{{\bf o}}
\def\pbf{{\bf p}}
\def\qbf{{\bf q}}
\def\rbf{{\bf r}}
\def\sbf{{\bf s}}
\def\tbf{{\bf t}}
\def\ubf{{\bf u}}
\def\vbf{{\bf v}}
\def\wbf{{\bf w}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\zbf{{\bf z}}
\def\rbf{{\bf r}}
\def\xbf{{\bf x}}
\def\ybf{{\bf y}}
\def\Abf{{\bf A}}
\def\Bbf{{\bf B}}
\def\Cbf{{\bf C}}
\def\Dbf{{\bf D}}
\def\Ebf{{\bf E}}
\def\Fbf{{\bf F}}
\def\Gbf{{\bf G}}
\def\Hbf{{\bf H}}
\def\Ibf{{\bf I}}
\def\Jbf{{\bf J}}
\def\Kbf{{\bf K}}
\def\Lbf{{\bf L}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Obf{{\bf O}}
\def\Pbf{{\bf P}}
\def\Qbf{{\bf Q}}
\def\Rbf{{\bf R}}
\def\Sbf{{\bf S}}
\def\Tbf{{\bf T}}
\def\Ubf{{\bf U}}
\def\Vbf{{\bf V}}
\def\Wbf{{\bf W}}
\def\Xbf{{\bf X}}
\def\Ybf{{\bf Y}}
\def\Zbf{{\bf Z}}
\def\Ac{{\cal A}}
\def\Bc{{\cal B}}
\def\Cc{{\cal C}}
\def\Dc{{\cal D}}
\def\Ec{{\cal E}}
\def\Fc{{\cal F}}
\def\Gc{{\cal G}}
\def\Hc{{\cal H}}
\def\Ic{{\cal I}}
\def\Jc{{\cal J}}
\def\Kc{{\cal K}}
\def\Lc{{\cal L}}
\def\Mc{{\cal M}}
\def\Nc{{\cal N}}
\def\Oc{{\cal O}}
\def\Pc{{\cal P}}
\def\Qc{{\cal Q}}
\def\Rc{{\cal R}}
\def\Sc{{\cal S}}
\def\Tc{{\cal T}}
\def\Uc{{\cal U}}
\def\Vc{{\cal V}}
\def\Wc{{\cal W}}
\def\Xc{{\cal X}}
\def\Yc{{\cal Y}}
\def\Zc{{\cal Z}}

\def\zsbf{{\boldsymbol{\mathsf z}}}
\def\wsbf{{\boldsymbol{\mathsf w}}}
\def\psbf{{\boldsymbol{\mathsf p}}}
\def\qsbf{{\boldsymbol{\mathsf q}}}
\def\xsbf{{\boldsymbol{\mathsf x}}}
\def\ysbf{{\boldsymbol{\mathsf y}}}
\def\deltasf{{\mathsf \delta}}
\def\isf{{\mathsf i}}


\def\nn{\nonumber}
\def\beq{\begin{equation}}
\def\eeq{\end{equation}}
\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}
\def\balign{\begin{align}}
\def\ealign{\end{align}}
\def\bpr{\begin{proof}}
\def\epr{\end{proof}}
\def\bth{\begin{theorem}}
\def\eth{\end{theorem}}
\def\blm{\begin{lemma}}
\def\elm{\end{lemma}}
\def\bprop{\begin{proposition}}
\def\eprop{\end{proposition}}
\def\bcr{\begin{corollary}}
\def\ecr{\end{corollary}}


\def\ie{{i.e.,\ \/}}
\def\eg{{\it e.g.,\ \/}}
\def\defeq{\triangleq}
\def\tr{{\rm tr}}
\def\vector{{\rm vec}}
\def\opt{{\rm opt}}
\def\st {{\rm subject~to~}}
\def\E{\mathbb{E}}
\def\gb{\succeq}
\def\gs{\preceq}
\def\rank{{\rm rank}}
\def\find {{\rm find}}
\def\tcb{\textcolor{Periwinkle}} %
\def\tcr{\textcolor{RubineRed}}
\def\and {{\rm and}}
\def\for {{\rm for~all}}

\newcommand{\fun}{f}
\newcommand{\pdf}{p}
\newcommand{\cdf}{F}
\newcommand{\ql}{\ell}
\newcommand{\bql}{{\boldsymbol \ell}}
\newcommand{\level}[1]{{\tau(#1)}}
\newcommand{\levelt}[1]{{\tilde \ql(#1)}}
\newcommand{\qcoeff}{{\rho}}
\newcommand{\feasl}{{\Lc}}
\newcommand{\rsym}{{\theta}}  %
\newcommand{\onesol}{{\beta}}
\DeclareMathOperator{\sign}{sign}
\newcommand{\signvec}{{\sbf}}
\newcommand{\dxdy}[2]{{\frac{\partial {#1}}{\partial {#2}}}} %
\newcommand{\dpsidl}{{\dxdy{\Psi(\bql(t))}{\ql_{j}}}}

\newcommand{\sgd}{{SGD}\xspace}
\newcommand{\supersgd}{{SuperSGD}\xspace}
\newcommand{\qinf}{{QSGDinf}\xspace}
\newcommand{\terngrad}{{TRN}\xspace}
\newcommand{\nuq}{{NUQSGD}\xspace}
\newcommand{\alqgnbased}{{ALQG}\xspace}
\newcommand{\alqgnless}{{ALQG-N}\xspace}
\newcommand{\alqnbased}{{ALQ}\xspace}
\newcommand{\amqnbased}{{AMQ}\xspace}
\newcommand{\alqnless}{{ALQ-N}\xspace}
\newcommand{\amqnless}{{AMQ-N}\xspace}
\newcommand{\op}{{overparameterization}\xspace}
\newcommand{\Op}{{Overparameterization}\xspace}
\newcommand{\oped}{{overparameterized}\xspace}

\newcommand{\med}{\mathrm{med}}
\newcommand{\Ag}{\mathrm{AGG}}
\newcommand{\nByz}{f}
\newcommand{\nAll}{n}

\DeclarePairedDelimiterX{\braket}[2]{\langle}{\rangle}{#1,#2}		%
\newcommand{\dual}[1]{#1^{\ast}}		%

\newcommand{\dspace}{\dual\vecspace}		%
\newcommand{\dvec}{\debug v}		%
\newcommand{\dbvec}{\debug \eps}		%
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert} 
\newcommand{\EG}{{EG}\xspace}
\newcommand{\GEG}{{GEG}\xspace}
\newcommand{\QEG}{{Q-GenX}\xspace}


\DeclareMathOperator{\Opt}{Opt}		%
\DeclareMathOperator{\Sol}{Sol}		%
\DeclareMathOperator{\gap}{Gap}         %

\newcommand{\points}{\mathcal{\debug X}}		%
\newcommand{\point}{\debug x}		%
\newcommand{\pointalt}{\alt\point}		%

\newcommand{\dpoints}{\mathcal{\debug y}}		%
\newcommand{\dpoint}{\debug y}		%
\newcommand{\dpointalt}{\alt\dpoint}		%
\newcommand{\obj}{\debug f}		%
\newcommand{\sobj}{\debug F}		%
\newcommand{\oper}{\debug A}		%


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
